Implicit Grid Convolution for Multi-Scale Image Super-Resolution

For Image Super-Resolution (SR), it is common to train and evaluate scale-specific models composed of an encoder and upsampler for each targeted scale. Consequently, many SR studies encounter substantial training times and complex deployment requirements. In this paper, we address this limitation by training and evaluating multiple scales simultaneously. Notably, we observe that encoder features are similar across scales and that the Sub-Pixel Convolution (SPConv), widely-used scale-specific upsampler, exhibits strong inter-scale correlations in its functionality. Building on these insights, we propose a multi-scale framework that employs a single encoder in conjunction with Implicit Grid Convolution (IGConv), our novel upsampler, which unifies SPConv across all scales within a single module. Extensive experiments demonstrate that our framework achieves comparable performance to existing fixed-scale methods while reducing the training budget and stored parameters three-fold and maintaining the same latency. Additionally, we propose IGConv$^{+}$ to improve performance further by addressing spectral bias and allowing input-dependent upsampling and ensembled prediction. As a result, ATD-IGConv$^{+}$ achieves a notable 0.21dB improvement in PSNR on Urban100$\times$4, while also reducing the training budget, stored parameters, and inference cost compared to the existing ATD.

==> Tab/main_quantitative.tex <==
\newcommand{\oc}{\cellcolor{orange}}

\begin{table*}[h!]
\caption{
    Comparisons of fixed-scale decoders and our proposed methods on various encoders. SPConv$^{+}$ denotes capacity-enhanced SPConv that additional convolution is employed after the pixel-shuffle operation of SPConv.
}\label{tab:fixedscale}
% \renewcommand{\arraystretch}{0.7}
\setlength{\extrarowheight}{0.2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ll|ccccc}
Dataset & Scale & \begin{tabular}[c]{@{}l@{}}Encoder \\ [-0.8ex] (Operator)\end{tabular} & Decoder & Set5 & Set14 & B100 & Urban100 & Manga109 \\ [-0.4ex] \hline
\multirow{27}{*}[5ex]{DIV2K} & \multirow{9}{*}[1.5ex]{2} & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}EDSR\\ (CNN)\end{tabular}} & SPConv$^{+}$ & 38.11/0.9602 & 33.92/0.9195 & 32.32/0.9013 & 32.93/0.9351 & 39.10/0.9773 \\ [-0.4ex]
 &  &  & IGConv & 38.21/0.9612 & 33.96/0.9209 & 32.34/0.9016 & 32.94/0.9359 & 39.13/0.9780 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 38.24/0.9614 & 33.96/0.9209 & 32.34/0.9018 & 33.00/0.9360 & 39.25/0.9783 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}HiT-SRF\\ (Transformer)\end{tabular}} & SPConv & 38.26/0.9615 & 34.01/0.9214 & 32.37/0.9023 & 33.13/0.9372 & 39.47/0.9787 \\ [-0.4ex]
 &  &  & IGConv & 38.16/0.9604 & 34.02/0.9214 & 32.35/0.9020 & 33.21/0.9377 & 39.34/0.9781 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 38.30/0.9615 & 33.97/0.9210 & 32.38/0.9023 & 33.22/0.9377 & 39.47/0.9786 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}MambaIR-light\\ (SSM)\end{tabular}} & SPConv & 38.16/0.9610 & 34.00/0.9212 & 32.34/0.9017 & 32.92/0.9356 & 39.31/0.9779 \\ [-0.4ex]
 &  &  & IGConv & 38.20/0.9611 & 34.02/0.9214 & 32.34/0.9014 & 33.02/0.9365 & 39.28/0.9782 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 38.20/0.9613 & 34.11/0.9221 & 32.36/0.9019 & 33.18/0.9372 & 39.44/0.9786 \\ [-0.4ex] \cline{2-9} 
 & \multirow{9}{*}[1.5ex]{3} & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}EDSR\\ (CNN)\end{tabular}} & SPConv$^{+}$ & 34.65/0.9280 & 30.52/0.8462 & 29.25/0.8093 & 28.80/0.8653 & 34.17/0.9476 \\ [-0.4ex]
 &  &  & IGConv & 34.70/0.9294 & 30.56/0.8469 & 29.28/0.8097 & 28.90/0.8671 & 34.31/0.9491 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 34.74/0.9298 & 30.65/0.8481 & 29.30/0.8103 & 28.95/0.8675 & 34.47/0.9496\\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}HiT-SRF\\ (Transformer)\end{tabular}} & SPConv & 34.75/0.9300 & 30.61/0.8475 & 29.29/0.8106 & 28.99/0.8687 & 34.53/0.9502 \\ [-0.4ex]
 &  &  & IGConv & 34.69/0.9292 & 30.60/0.8476 & 29.26/0.8098 & 29.02/0.8694 & 34.46/0.9499 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 34.78/0.9302 & 30.69/0.8488 & 29.32/0.8111 & 29.06/0.8693 & 34.67/0.9506 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}MambaIR-light\\ (SSM)\end{tabular}} & SPConv & 34.72/0.9296 & 30.63/0.8475 & 29.29/0.8099 & 29.00/0.8689 & 34.39/0.9495 \\ [-0.4ex]
 &  &  & IGConv & 34.70/0.9294 & 30.59/0.8474 & 29.27/0.8094 & 28.91/0.8672 & 34.37/0.9492 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 34.74/0.9298 & 30.68/0.8487 & 29.30/0.8105 & 29.04/0.8687 & 34.62/0.9502 \\ [-0.4ex] \cline{2-9} 
 & \multirow{9}{*}[1.5ex]{4} & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}EDSR\\ (CNN)\end{tabular}} & SPConv$^{+}$ & 32.46/0.8968 & 28.80/0.7876 & 27.71/0.7420 & 26.64/0.8033 & 31.02/0.9148 \\ [-0.4ex]
 &  &  & IGConv & 32.57/0.8990 & 28.84/0.7880 & 27.76/0.7426 & 26.75/0.8060 & 31.29/0.9178 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 32.59/0.8996 & 28.91/0.7890 & 27.79/0.7433 & 26.82/0.8064 & 31.43/0.9182 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}HiT-SRF\\ (Transformer)\end{tabular}} & SPConv & 32.55/0.8999 & 28.87/0.7880 & 27.75/0.7432 & 26.80/0.8069 & 31.26/0.9171 \\ [-0.4ex]
 &  &  & IGConv & 32.53/0.8988 & 28.90/0.7887 & 27.71/0.7422 & 26.88/0.8085 & 31.31/0.9184 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 32.60/0.9001 & 28.95/0.7892 & 27.80/0.7440 & 26.91/0.8083 & 31.57/0.9198 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}MambaIR-light\\ (SSM)\end{tabular}} & SPConv & 32.51/0.8993 & 28.85/0.7876 & 27.75/0.7423 & 26.75/0.8051 & 31.26/0.9175 \\ [-0.4ex]
 &  &  & IGConv & 32.50/0.8992 & 28.86/0.7879 & 27.75/0.7422 & 26.72/0.8045 & 31.29/0.9175 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 32.62/0.8997 & 28.93/0.7893 & 27.80/0.7437 & 26.87/0.8068 & 31.51/0.9185 \\ [-0.4ex] \hline
\multirow{27}{*}[5ex]{DF2K} & \multirow{9}{*}[1.5ex]{2} & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}SMFANet+\\ (CNN)\end{tabular}} & SPConv & 38.19/0.9611 & 33.92/0.9207 & 32.32/0.9015 & 32.70/0.9331 & 39.46/0.9787 \\ [-0.4ex]
 &  &  & IGConv & 38.16/0.9610 & 33.96/0.9213 & 32.32/0.9014 & 32.73/0.9332 & 39.38/0.9785 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 38.14/0.9611 & 33.92/0.9208 & 32.32/0.9014 & 32.76/0.9334 & 39.40/0.9786 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}SRFormer\\ (Transformer)\end{tabular}} & SPConv$^{+}$ & 38.51/0.9627 & 34.44/0.9253 & 32.57/0.9046 & 34.09/0.9449 & 40.07/0.9802 \\ [-0.4ex]
 &  &  & IGConv & 38.44/0.9625 & 34.64/0.9267 & 32.56/0.9048 & 34.28/0.9462 & 39.88/0.9798 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 38.53/0.9626 & 34.72/0.9268 & 32.60/0.9052 & 34.42/0.9468 & 40.03/0.9797 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}MambaIR\\ (SSM)\end{tabular}} & SPConv$^{+}$ & 38.57/0.9627 & 34.67/0.9261 & 32.58/0.9048 & 34.15/0.9446 & 40.28/0.9806 \\ [-0.4ex]
 &  &  & IGConv & 38.48/0.9624 & 34.68/0.9264 & 32.58/0.9047 & 34.26/0.9453 & 40.14/0.9803 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 38.55/0.9625 & 34.81/0.9270 & 32.62/0.9052 & 34.37/0.9461 & 40.19/0.9802 \\ [-0.4ex] \cline{2-9} 
 & \multirow{9}{*}[1.5ex]{3} & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}SMFANet+\\ (CNN)\end{tabular}} & SPConv & 34.66/0.9292 & 30.57/0.8461 & 29.25/0.8090 & 28.67/0.8611 & 34.45/0.9490 \\ [-0.4ex]
 &  &  & IGConv & 34.62/0.9290 & 30.56/0.8461 & 29.25/0.8090 & 28.64/0.8606 & 34.45/0.9490 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 34.62/0.9290 & 30.56/0.8461 & 29.25/0.8090 & 28.64/0.8606 & 34.45/0.9490 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}SRFormer\\ (Transformer)\end{tabular}} & SPConv$^{+}$ & 35.02/0.9323 & 30.94/0.8540 & 29.48/0.8156 & 30.04/0.8865 & 35.26/0.9543 \\ [-0.4ex]
 &  &  & IGConv & 34.96/0.9323 & 30.95/0.8543 & 29.47/0.8157 & 30.11/0.8876 & 35.16/0.9543 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 35.08/0.9329 & 31.06/0.8551 & 29.52/0.8166 & 30.25/0.8888 & 35.45/0.9550 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}MambaIR\\ (SSM)\end{tabular}} & SPConv$^{+}$ & 35.08/0.9323 & 30.99/0.8536 & 29.51/0.8157 & 29.93/0.8841 & 35.43/0.9546 \\ [-0.4ex]
 &  &  & IGConv & 35.04/0.9320 & 31.01/0.8535 & 29.50/0.8154 & 29.95/0.8844 & 35.44/0.9545 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 35.10/0.9325 & 31.14/0.8550 & 29.55/0.8164 & 30.11/0.8864 & 35.55/0.9549 \\ [-0.4ex] \cline{2-9} 
 & \multirow{9}{*}[1.5ex]{4} & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}SMFANet+\\ (CNN)\end{tabular}} & SPConv & 32.51/0.8985 & 28.87/0.7872 & 27.74/0.7412 & 26.56/0.7976 & 31.29/0.9163 \\ [-0.4ex]
 &  &  & IGConv & 32.47/0.8982 & 28.84/0.7866 & 27.74/0.7413 & 26.54/0.7969 & 31.28/0.9158 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 32.52/0.8988 & 28.83/0.7867 & 27.74/0.7413 & 26.55/0.7974 & 31.29/0.9161 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}SRFormer\\ (Transformer)\end{tabular}} & SPConv$^{+}$ & 32.93/0.9041 & 29.08/0.7953 & 27.94/0.7502 & 27.68/0.8311 & 32.21/0.9271 \\ [-0.4ex]
 &  &  & IGConv & 32.87/0.9046 & 29.08/0.7952 & 27.91/0.7499 & 27.79/0.8333 & 32.14/0.9274 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 33.04/0.9047 & 29.22/0.7971 & 27.99/0.7509 & 27.93/0.8350 & 32.45/0.9288 \\ [-0.4ex] \cline{3-9} 
 &  & \multirow{3}{*}[0.3ex]{\begin{tabular}[c]{@{}l@{}}MambaIR\\ (SSM)\end{tabular}} & SPConv$^{+}$ & 33.03/0.9046 & 29.20/0.7961 & 27.98/0.7503 & 27.68/0.8287 & 32.32/0.9272 \\ [-0.4ex]
 &  &  & IGConv & 32.98/0.9041 & 29.17/0.7955 & 27.97/0.7498 & 27.68/0.8288 & 32.36/0.9271 \\ [-0.4ex]
 &  &  & IGConv$^{+}$ & 33.05/0.9045 & 29.25/0.7969 & 28.02/0.7512 & 27.80/0.8314 & 32.52/0.9280 \\ [-0.4ex] \hline
\end{tabular}
}
\end{table*}

% \begin{table*}[ht!]
% \caption{
%     Comparisons of SPConv and our proposed methods on various encoders. SPConv$^{+}$ denotes capacity-enhanced SPConv that additional convolution is employed after the pixel-shuffle operation of SPConv.
% }\label{tab:fixedscale}
% \renewcommand{\arraystretch}{0.6}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|llll|ccccc}
% Scale & Operator & Encoder & Dataset & Decoder & Set5 & Set14 & B100 & Urban100 & Manga109 \\ \hline
% \multirow{18}{*}{2} & \multirow{6}{*}{CNN} & \multirow{3}{*}{EDSR} & \multirow{3}{*}{DIV2K} & SPConv$^{+}$ & 38.11/0.9602 & 33.92/0.9195 & 32.32/0.9013 & 32.93/0.9351 & 39.10/0.9773 \\
%  &  &  &  & IGConv & 38.21/0.9612 & 33.96/0.9209 & 32.34/0.9016 & 32.94/0.9359 & 39.13/0.9780 \\
%  &  &  &  & IGConv$^{+}$ & 38.24/0.9614 & 33.96/0.9209 & 32.34/0.9018 & 33.00/0.9360 & 39.25/0.9783 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{SMFANet+} & \multirow{3}{*}{DF2K} & SPConv & 38.19/0.9611 & 33.92/0.9207 & 32.32/0.9015 & 32.70/0.9331 & 39.46/0.9787 \\
%  &  &  &  & IGConv & 38.16/0.9610 & 33.96/0.9213 & 32.32/0.9014 & 32.73/0.9332 & 39.38/0.9785 \\
%  &  &  &  & IGConv$^{+}$ & 38.14/0.9611 & 33.92/0.9208 & 32.32/0.9014 & 32.76/0.9334 & 39.40/0.9786 \\ \cline{2-10} 
%  & \multirow{6}{*}{Transformer} & \multirow{3}{*}{HiT-SRF} & \multirow{3}{*}{DIV2K} & SPConv & 38.26/0.9615 & 34.01/0.9214 & 32.37/0.9023 & 33.13/0.9372 & 39.47/0.9787 \\
%  &  &  &  & IGConv & 38.16/0.9604 & 34.02/0.9214 & 32.35/0.9020 & 33.21/0.9377 & 39.34/0.9781 \\
%  &  &  &  & IGConv$^{+}$ & 38.30/0.9615 & 33.97/0.9210 & 32.38/0.9023 & 33.22/0.9377 & 39.47/0.9786 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{SRFormer} & \multirow{3}{*}{DF2K} & SPConv$^{+}$ & 38.51/0.9627 & 34.44/0.9253 & 32.57/0.9046 & 34.09/0.9449 & 40.07/0.9802 \\
%  &  &  &  & IGConv & 38.44/0.9625 & 34.64/0.9267 & 32.56/0.9048 & 34.28/0.9462 & 39.88/0.9798 \\
%  &  &  &  & IGConv$^{+}$ & 38.53/0.9626 & 34.72/0.9268 & 32.60/0.9052 & 34.42/0.9468 & 40.03/0.9797 \\ \cline{2-10} 
%  & \multirow{6}{*}{SSM} & \multirow{3}{*}{MambaIR-light} & \multirow{3}{*}{DIV2K} & SPConv & 38.16/0.9610 & 34.00/0.9212 & 32.34/0.9017 & 32.92/0.9356 & 39.31/0.9779 \\
%  &  &  &  & IGConv & 38.20/0.9611 & 34.02/0.9214 & 32.34/0.9014 & 33.02/0.9365 & 39.28/0.9782 \\
%  &  &  &  & IGConv$^{+}$ & 38.20/0.9613 & 34.11/0.9221 & 32.36/0.9019 & 33.18/0.9372 & 39.44/0.9786 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{MambaIR} & \multirow{3}{*}{DF2K} & SPConv$^{+}$ & 38.57/0.9627 & 34.67/0.9261 & 32.58/0.9048 & 34.15/0.9446 & 40.28/0.9806 \\
%  &  &  &  & IGConv & 38.48/0.9624 & 34.68/0.9264 & 32.58/0.9047 & 34.26/0.9453 & 40.14/0.9803 \\
%  &  &  &  & IGConv$^{+}$ & 38.55/0.9625 & 34.81/0.9270 & 32.62/0.9052 & 34.37/0.9461 & 40.19/0.9802 \\ \hline
% \multirow{18}{*}{3} & \multirow{6}{*}{CNN} & \multirow{3}{*}{EDSR} & \multirow{3}{*}{DIV2K} & SPConv$^{+}$ & 34.65/0.9280 & 30.52/0.8462 & 29.25/0.8093 & 28.80/0.8653 & 34.17/0.9476 \\
%  &  &  &  & IGConv & 34.70/0.9294 & 30.56/0.8469 & 29.28/0.8097 & 28.90/0.8671 & 34.31/0.9491 \\
%  &  &  &  & IGConv$^{+}$ & 34.74/0.9298 & 30.65/0.8481 & 29.30/0.8103 & 28.95/0.8675 & 34.47/0.9496 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{SMFANet+} & \multirow{3}{*}{DF2K} & SPConv & 34.66/0.9292 & 30.57/0.8461 & 29.25/0.8090 & 28.67/0.8611 & 34.45/0.9490 \\
%  &  &  &  & IGConv & 34.62/0.9290 & 30.56/0.8461 & 29.25/0.8090 & 28.64/0.8606 & 34.45/0.9490 \\
%  &  &  &  & IGConv$^{+}$ & 34.58/0.9287 & 30.58/0.8464 & 29.24/0.8089 & 28.66/0.8610 & 34.45/0.9490 \\ \cline{2-10} 
%  & \multirow{6}{*}{Transformer} & \multirow{3}{*}{HiT-SRF} & \multirow{3}{*}{DIV2K} & SPConv & 34.75/0.9300 & 30.61/0.8475 & 29.29/0.8106 & 28.99/0.8687 & 34.53/0.9502 \\
%  &  &  &  & IGConv & 34.69/0.9292 & 30.60/0.8476 & 29.26/0.8098 & 29.02/0.8694 & 34.46/0.9499 \\
%  &  &  &  & IGConv$^{+}$ & 34.78/0.9302 & 30.69/0.8488 & 29.32/0.8111 & 29.06/0.8693 & 34.67/0.9506 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{SRFormer} & \multirow{3}{*}{DF2K} & SPConv$^{+}$ & 35.02/0.9323 & 30.94/0.8540 & 29.48/0.8156 & 30.04/0.8865 & 35.26/0.9543 \\
%  &  &  &  & IGConv & 34.96/0.9323 & 30.95/0.8543 & 29.47/0.8157 & 30.11/0.8876 & 35.16/0.9543 \\
%  &  &  &  & IGConv$^{+}$ & 35.08/0.9329 & 31.06/0.8551 & 29.52/0.8166 & 30.25/0.8888 & 35.45/0.9550 \\ \cline{2-10} 
%  & \multirow{6}{*}{SSM} & \multirow{3}{*}{MambaIR-light} & \multirow{3}{*}{DIV2K} & SPConv & 34.72/0.9296 & 30.63/0.8475 & 29.29/0.8099 & 29.00/0.8689 & 34.39/0.9495 \\
%  &  &  &  & IGConv & 34.70/0.9294 & 30.59/0.8474 & 29.27/0.8094 & 28.91/0.8672 & 34.37/0.9492 \\
%  &  &  &  & IGConv$^{+}$ & 34.74/0.9298 & 30.68/0.8487 & 29.30/0.8105 & 29.04/0.8687 & 34.62/0.9502 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{MambaIR} & \multirow{3}{*}{DF2K} & SPConv$^{+}$ & 35.08/0.9323 & 30.99/0.8536 & 29.51/0.8157 & 29.93/0.8841 & 35.43/0.9546 \\
%  &  &  &  & IGConv & 35.04/0.9320 & 31.01/0.8535 & 29.50/0.8154 & 29.95/0.8844 & 35.44/0.9545 \\
%  &  &  &  & IGConv$^{+}$ & 35.10/0.9325 & 31.14/0.8550 & 29.55/0.8164 & 30.11/0.8864 & 35.55/0.9549 \\ \hline
% \multirow{18}{*}{4} & \multirow{6}{*}{CNN} & \multirow{3}{*}{EDSR} & \multirow{3}{*}{DIV2K} & SPConv$^{+}$ & 32.46/0.8968 & 28.80/0.7876 & 27.71/0.7420 & 26.64/0.8033 & 31.02/0.9148 \\
%  &  &  &  & IGConv & 32.57/0.8990 & 28.84/0.7880 & 27.76/0.7426 & 26.75/0.8060 & 31.29/0.9178 \\
%  &  &  &  & IGConv$^{+}$ & 32.59/0.8996 & 28.91/0.7890 & 27.79/0.7433 & 26.82/0.8064 & 31.43/0.9182 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{SMFANet+} & \multirow{3}{*}{DF2K} & SPConv & 32.51/0.8985 & 28.87/0.7872 & 27.74/0.7412 & 26.56/0.7976 & 31.29/0.9163 \\
%  &  &  &  & IGConv & 32.47/0.8982 & 28.84/0.7866 & 27.74/0.7413 & 26.54/0.7969 & 31.28/0.9158 \\
%  &  &  &  & IGConv$^{+}$ & 32.52/0.8988 & 28.83/0.7867 & 27.74/0.7413 & 26.55/0.7974 & 31.29/0.9161 \\ \cline{2-10} 
%  & \multirow{6}{*}{Transformer} & \multirow{3}{*}{HiT-SRF} & \multirow{3}{*}{DIV2K} & SPConv & 32.55/0.8999 & 28.87/0.7880 & 27.75/0.7432 & 26.80/0.8069 & 31.26/0.9171 \\
%  &  &  &  & IGConv & 32.53/0.8988 & 28.90/0.7887 & 27.71/0.7422 & 26.88/0.8085 & 31.31/0.9184 \\
%  &  &  &  & IGConv$^{+}$ & 32.60/0.9001 & 28.95/0.7892 & 27.80/0.7440 & 26.91/0.8083 & 31.57/0.9198 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{SRFormer} & \multirow{3}{*}{DF2K} & SPConv$^{+}$ & 32.93/0.9041 & 29.08/0.7953 & 27.94/0.7502 & 27.68/0.8311 & 32.21/0.9271 \\
%  &  &  &  & IGConv & 32.87/0.9046 & 29.08/0.7952 & 27.91/0.7499 & 27.79/0.8333 & 32.14/0.9274 \\
%  &  &  &  & IGConv$^{+}$ & 33.04/0.9047 & 29.22/0.7971 & 27.99/0.7509 & 27.93/0.8350 & 32.45/0.9288 \\ \cline{2-10} 
%  & \multirow{6}{*}{SSM} & \multirow{3}{*}{MambaIR-light} & \multirow{3}{*}{DIV2K} & SPConv & 32.51/0.8993 & 28.85/0.7876 & 27.75/0.7423 & 26.75/0.8051 & 31.26/0.9175 \\
%  &  &  &  & IGConv & 32.50/0.8992 & 28.86/0.7879 & 27.75/0.7422 & 26.72/0.8045 & 31.29/0.9175 \\
%  &  &  &  & IGConv$^{+}$ & 32.62/0.8997 & 28.93/0.7893 & 27.80/0.7437 & 26.87/0.8068 & 31.51/0.9185 \\ \cline{3-10} 
%  &  & \multirow{3}{*}{MambaIR} & \multirow{3}{*}{DF2K} & SPConv$^{+}$ & 33.03/0.9046 & 29.20/0.7961 & 27.98/0.7503 & 27.68/0.8287 & 32.32/0.9272 \\
%  &  &  &  & IGConv & 32.98/0.9041 & 29.17/0.7955 & 27.97/0.7498 & 27.68/0.8288 & 32.36/0.9271 \\
%  &  &  &  & IGConv$^{+}$ & 33.05/0.9045 & 29.25/0.7969 & 28.02/0.7512 & 27.80/0.8314 & 32.52/0.9280 \\ \hline
% \end{tabular}%
% }
% \end{table*}


==> Tab/sota_ood.tex <==
\begin{table*}[]
\caption{
    Comparison of ASSR upsamplers with our proposal. Metrics are calculated by upsampling a 128$\times$128 image \textbf{at scale $\times$8} using an A6000 GPU.
}\label{tab:sota_ood}
\renewcommand{\arraystretch}{0.7}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|ccc|cc|cc|cc|cc}
\multirow{2}{*}{Encoder} & \multirow{2}{*}{Decoder} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Latency\\ (ms)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\#Params\\ (K)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Memory \\ (mb)\end{tabular}} & \multicolumn{2}{c}{Set5} & \multicolumn{2}{c}{Set14} & \multicolumn{2}{c}{B100} & \multicolumn{2}{c}{Urban100} \\
 &  &  &  &  & $\times$6 & $\times$8 & $\times$6 & $\times$8 & $\times$6 & $\times$8 & $\times$6 & $\times$8 \\ \hline

% RDN -------------------------------------------------------
\multirow{7}{*}{RDN} & LIIF & 639.5 & 347 & 7086 & 29.15 & 27.14 & 26.64 & 25.15 & 25.98 & 24.91 & 24.20 & 22.79 \\
 & LTE  & 668.7 & 494 & 6291 & 29.32 & 27.26 & 26.71 & 25.16 & 26.01 & 24.95 & 24.28 & 22.88 \\
 & CiaoSR & OOM & 1429 & OOM & 29.46 & 27.36 & 26.79 & 25.28 & 26.07 & 25.00 & 24.58 & 23.13 \\
 & LM-LTE & 89.4 & 271 & 1327 & 29.21 & 27.22 & 26.69 & 25.15 & 26.01 & 24.95 & 24.26 & 22.86 \\
 & OPE-SR & 55.3 & \textbf{0} & 1293 & 29.17 & 27.22 & 26.65 & 25.17 & 25.96 & 24.91 & 24.06 & 22.70 \\
 & CUF & - / 5.0$^{\S}$ & 10 & - / 516$^{\S}$  & 29.25 & - & 26.70 & - & 25.99 & - & 24.23 & - \\
 \highlightigconv & \textbf{IGConv$^{+}$} & \textbf{6.1} / \textbf{1.5}$^{\S}$ & 922 & \textbf{316} / \textbf{162}$^{\S}$  & 29.21 & 27.22 & 26.69 & 25.20 & 26.00 & 24.94 & 24.25 & 22.84 \\ \hline
 
% SwinIR -------------------------------------------------------
 \multirow{6}{*}{SwinIR} & LIIF & 1482.7 & 614 & 19688 &  29.46 & 27.36 & 26.82 & 25.34 & 26.07 & 25.01 & 24.59 & 23.14  \\
 & LTE & 670 & 1028 & 6300 & 29.50 & 27.35 & 26.86 & 25.42 & 26.09 & 25.03 & 24.62 & 23.17 \\
 & CiaoSR & OOM & 3168 & OOM & 29.62 & 27.45 & 26.88 & 25.42 & 26.13 & 25.07 & 24.84 & 23.34  \\
 & LM-LTE & 89.4 & 538 & 1336 & 29.52 & 27.39 & 26.83 & 25.38 & 26.10 & 25.03 & 24.63 & 23.17 \\ 
 & CUF & - / 14.1$^{\S}$ & \textbf{37} & - / 1453$^{\S}$ & 29.53 & - & 26.85 & - & 26.09 & - & 24.62 & -  \\
 \highlightigconv & \textbf{IGConv$^{+}$} & \textbf{15.8} / \textbf{2.3}$^{\S}$ & 1991 & \textbf{733} / 173$^{\S}$ & 29.39 & 27.34 & 26.80 & 25.35 & 26.07 & 25.02 & 24.55 & 23.10 \\ \hline
\end{tabular}%
}
\end{table*}

==> reviews.tex <==
% R1

1) What exactly does “implicit” refer to in Implicit Grid Convolution? Implicit representation typically describes objects or scenes continuously via functions. Does this conflict with the concept of a “grid”? 
Methods에서 설명하기

2) Methods like ArbSR [1] and EQSR [2] also explored the correlation between tasks at different scales during feature extraction, improving the discriminative learning capability of a single encoder across multiple scales by introducing scale information. However, the authors only demonstrated the similarity between scales in Figure 3 without addressing discriminative feature learning across different scales. Is this approach reasonable? 
일단 하나의 encoder를 사용하고 나서 생각해야 할 문제라고 써두기

3) In Appendix Table 9, the authors train the model on a limited number of integer scales and achieve arbitrary scale super-resolution through downsampling. Why not directly train the model for arbitrary scale tasks? Please explain the reasoning behind this design, and how it can achieve performance comparable to arbitrary scale upsampling methods. Additionally, the authors should compare their method with the latest arbitrary video super-resolution methods (e.g., ST-AVSR [R3], SAVSR [R4]) to validate its performance. 
설명 더 자세히쓰기
+ 비디오는 억까

4) Is the use of Fourier transform truly necessary for a hypernetwork with only a few scale inputs? Fourier transforms are typically effective when the data exhibit periodic or frequency-based characteristics. Were its multi-scale and frequency-capturing capabilities fully utilized in cases with limited scales (e.g., ×2, ×3, ×4)? Would it be simpler and more effective to generate convolutional kernels directly in the spatial domain? 
단순히 input을 fourier basis로 던지는 것 만으로도 spectral bias를 줄일 수 있다는 연구를 따랐다.
또한 최근 Burst Image Super-Resolution domain의 연구도 2, 3, 4만 학습하더라도 fourier basis를 사용하는 것이 성능 향상에 주요했다고 언급.
더 나아가 연구에서는 2, 3, 4만 하지만 실제로는 더 많은 scale을 고려할 수 잇고 이런 상황에서는 큰 도움이 될 것 같다.

5) The method has demonstrated the correlation between different scales through experiments and visualizations. Can it be directly extended to large-scale upsampling tasks (e.g., ×24, ×30 as mentioned in LIIF)? 
서플에 넣기 (잘안된다)

6) The introduction mentions, “Our extensive experiments demonstrate that multi-scale training with IGConv reduces the training budget and stored parameters by one-third while maintaining or improving performance compared to models trained on a fixed scale.” Please compare the performance of the proposed method with models trained on fixed scales. 
hyper-network를 사용하지 않고 fixed-scale을 학습하면 그냥 SPConv를 사용하는 것과 같음. 
이런 차이점을 자세히 써주기

7) Figure 1 is not cited or explained in the main text, and there is a typo in the title of Figure 4. 
고치기

8) The function of the model is insufficient and the code is unavailable for verification.
고치기

% R2

It is necessary to show the training cost of the proposed method compared to the single scale model. This is helpful to understand the advantages and disadvantages of the proposed method.
Table 추가

The proposed method uses stronger training strategies such as frequency loss. Moreover, the extra parameters brought by IGConv cannot be ignored for lightweight models. The performance gain may originate from this. Additional experiments are needed to compare the performance of IGConv and single scale models with the same parameters.
Ablation 보면 Frequency 이외의 다른 애들도 성능 향상에 큰 기여를 한다.
Structrual Re-parameterization처럼 결국 같은 operation이 되거나 더 적은 parameter를 가지게된다고 설명

All tests were performed on the lightweight model. The authors need to evaluate the validity of the method on some larger methods.
ATD, HAT 실험 추가

Comparisons with other arbitrary scale SR models need to be included in the main text as it is very relevant to the proposed methodology.
...

